ShuttleSHAP: A Turn-Based Feature Attribution Approach for Analyzing Forecasting Models in Badminton

Agent forecasting systems have been explored to investigate agent patterns and improve decision-making in various domains, e.g., pedestrian predictions and marketing bidding. Badminton represents a fascinating example of a multifaceted turn-based sport, requiring both sophisticated tactic developments and alternate-dependent decision-making. Recent deep learning approaches for player tactic forecasting in badminton show promising performance partially attributed to effective reasoning about rally-player interactions. However, a critical obstacle lies in the unclear functionality of which features are learned for simulating players' behaviors by black-box models, where existing explainers are not equipped with turn-based and multi-output attributions. To bridge this gap, we propose a turn-based feature attribution approach, ShuttleSHAP, for analyzing forecasting models in badminton based on variants of Shapley values. ShuttleSHAP is a model-agnostic explainer that aims to quantify contribution by not only temporal aspects but also player aspects in terms of multifaceted cues. Incorporating the proposed analysis tool into the state-of-the-art turn-based forecasting model on the benchmark dataset reveals that it is, in fact, insignificant to reason about past strokes, while conventional sequential models have greater impacts. Instead, players' styles influence the models for the future simulation of a rally. On top of that, we investigate and discuss the causal analysis of these findings and demonstrate the practicability with local analysis.

==> tables/match-info.tex <==
\begin{tabular}{cccc}
    \toprule
    Tournament & Round \\
    \midrule
    Fuzhou Open 2018 & Finals \\
    Denmark Open 2018 & Finals \\
    Malaysia Open 2018 & Quarter-finals \\
    Asia Championships 2018 & Quarter-finals \\
    Fuzhou Open 2019 & Semi-finals \\
    Fuzhou Open 2019 & Finals \\
    Hong Kong Open 2019 & Quarter-finals \\
    World Tour Finals & Group-Stage \\
    Korea Open 2019 & Finals \\
    Denmark Open 2019 & Quarter-finals \\
    China Open 2019 & Quarter-finals \\
    Indonesia Open 2019 & Finals \\
    World Tour Finals 2019 & Group-Stage \\
    World Tour Finals 2019 & Semi-finals \\
    World Tour Finals 2019 & Finals \\
    World Championships 2019 & Quarter-finals \\
    Denmark Open 2019 & Round-of-32 \\
    Sudirman Cup 2019 & Quarter-finals \\
    Sudirman Cup 2019 & Group-Stage \\
    Indonesia Open 2019 & Quarter-finals \\
    All England Open 2020 & Quarter-finals \\
    All England Open 2020 & Finals \\
    Thailand Masters 2020 & Semi-finals \\
    Indonesia Masters 2020 & Quarter-finals \\
    Indonesia Masters 2020 & Semi-finals \\
    Indonesia Masters 2020 & Finals \\
    Malaysia Masters 2020 & Round-of-16 \\
    Malaysia Masters 2020 & Quarter-finals \\
    Malaysia Masters 2020 & Semi-finals \\
    Malaysia Masters 2020 & Finals \\
    YONEX Thailand Open 2021 & Quarter-finals \\
    YONEX Thailand Open 2021 & Semi-finals \\
    YONEX Thailand Open 2021 & Finals \\
    TOYOTA Thailand Open 2021 & Quarter-finals \\
    TOYOTA Thailand Open 2021 & Semi-finals \\
    TOYOTA Thailand Open 2021 & Finals \\
    HSBC BWF World Tour Finals 2020 & Group-Stage \\
    HSBC BWF World Tour Finals 2020 & Quarter-finals \\
    HSBC BWF World Tour Finals 2020 & Semi-finals \\
    HSBC BWF World Tour Finals 2020 & Finals \\
    \bottomrule
\end{tabular}

==> tables/shot-type-descriptions.tex <==
\begin{tabular}{c|l}
    \toprule
    Shot type       & Description \\
    \midrule
    net shot        & A soft shot that places the shuttle close to the net.\\
    \midrule
    smash           & A fast, downward angled shot that is performed with an overhand motion. \\
    \midrule
    lob       & \makecell[l]{A defensive shot that is typically performed from the front of the court by pushing the shuttle high and \\ far to the back of the opponent’s end of the court.} \\
    \midrule
    clear & A high overhand shot where the player hits the shuttle from one end of the court to the other end. \\
    \midrule
    drive & \makecell[l]{A fast and flat shot that travels just above the net, which is used for both offensive and defensive \\ purposes.}\\
    \midrule
    drop & \makecell[l]{An active shot that places the shuttle close to the net, often in an attempt to make the opponent move or \\ to set up for the next shot.}\\
    \midrule
    push/rush       & A shot pushed/rushed from near the net to land at the back court for landing quickly.\\
    \midrule
    defensive shot  & A shot that returns the smash from the middle or back court of the opponent to the middle or back court. \\
    \midrule
    short service   & A serve that goes over the top of the net and lands near the short service line.\\
    \midrule
    long service    & A serve that goes high and deep into the opponent’s back court.\\
    \bottomrule
\end{tabular}
